Beyond Confusion: A Fine-grained Dialectical Examination of Human Activity Recognition Benchmark Datasets

The research of machine learning (ML) algorithms for human activity recognition (HAR) has made significant progress with publicly available datasets. However, most research prioritizes statistical metrics over examining negative sample details. While recent models like transformers have been applied to HAR datasets with limited success from the benchmark metrics, their counterparts have effectively solved problems on similar levels with near 100% accuracy. This raises questions about the limitations of current approaches. This paper aims to address these open questions by conducting a fine-grained inspection of six popular HAR benchmark datasets. We identified for some parts of the data, none of the six chosen state-of-the-art ML methods can correctly classify, denoted as the intersect of false classifications (IFC). Analysis of the IFC reveals several underlying problems, including ambiguous annotations, irregularities during recording execution, and misaligned transition periods. We contribute to the field by quantifying and characterizing annotated data ambiguities, providing a trinary categorization mask for dataset patching, and stressing potential improvements for future data collections.

==> sections/x_oldrelatedwork.tex <==

%The \textit{Skoda} dataset (2008) \cite{zappi2008activity} captures 10  manipulative gestures in a car maintenance scenario from a single participant, recorded using 20 three-axis accelerometers placed on both arms.

The \textit{HCI gestures} dataset (2009) \cite{forster2009unsupervised} five gestures performed by a single participant freehand or against a blackboard with eight 3-axis accelerometers on a single arm, mainly to evaluate the effect of sensor displacement.

The \textit{WISDM} dataset (2011) \cite{kwapisz2011wisdm} contains accelerometer recordings from a smartphone in the pocket with 29 participants performing six daily locomotion activities.

The \textit{HASC} dataset (2011) \cite{hasc2011} is a large-scale data collection effort with 540 participants performing six daily locomotion activities.

The \textit{Darmstadt Daily Routines} dataset (2011) \cite{plotz2011feature}

The \textit{PAMAP2} dataset (2012) \cite{reiss2012pamap2} consists of over 10 hours of recordings in total from nine participants performing 18 daily living activities, captured using a heart rate monitor and three 9-axis IMUs on the chest, dominant wrist, and dominant ankle. %comprises recordings from nine participants performing 18 activities of daily living, totaling over 10 hours of data. It includes one heart rate-monitor channel and three Inertial Measurement Units (IMUs) placed on the subject's chest, dominant wrist, and dominant ankle, yielding a dataset with 52 channels. Each IMU contains 17 channels, including acceleration, gyroscope, magnetometer, and orientation data.

The \textit{RealDisp} dataset (2012) \cite{banos2012benchmark} recorded 9 hours of daily activity data from 17 volunteers, involving 33 activities encompassing whole-body movements and body part-specific actions such as walking, jogging, cycling, and bending. It includes data from 9 IMUs distributed across various body parts.

The \textit{Daphnet} dataset (2012) \cite{durka2012daphne}

The \textit{Opportunity} dataset (2013) \cite{chavarriaga2013opportunity} contains 6 hours of data recordings from four participants performing daily activities wearing seven 9-axis IMUs and 12 additional 3-axis accelerometers. It was annotated on different levels of granularity, with one label track for five locomotion classes, one track for five high level activities (e.g. making breakfast), and one track for 18 atomic gestures (e.g. open drawer 2). % with two separate tracks of five modes of locomotion and 18 gestures, . % from wearable, object, and ambient sensors, featuring data;  With a total of  recordings and a sampling frequency of $\SI{30}{\hertz}$, it includes body-worn sensors with 145 channels, object sensors with 60 channels, and ambient sensors with 37 channels.
The \textit{Opportunity++} dataset (2021) \cite{ciliberto2021opportunity++}
includes anatomized videos and full-body poses from the 2013 experiment.

The \textit{UCI-HAR} dataset (2013) \cite{anguita2013public} records six daily locomotion activities using accelerometers and gyroscopes embedded in a waist-attached smartphone from 30 participants.
% Thirty volunteers, aged 19 to 48, participated in the data collection phase with the phone attached to their waists, capturing 3-axial linear acceleration and 3-axial angular velocity at a constant rate of $\SI{50}{\hertz}$.

The \textit{MHealth} dataset (2014) \cite{banos2014mhealth} collected data from 10 volunteers performing 12 fitness-focused physical activities each recorded for a minute or repeated 20 times while wearing 3 IMUs on the chest, left ankle, and right lower arm, together with one 2-lead ECG sensor.  %, including climbing stairs, walking, waist bends forward, and cycling. It includes measurements from three IMUs and a chest sensor providing 2-lead ECG data, all sampled at $\SI{50}{\hertz}$. 

The \textit{USC-HAD} dataset (2015) \cite{jiang2015human}

The \textit{DSADS} dataset (2015) \cite{zhang2015recognizing} involves 19 activities, executed by eight subjects, with data captured from five IMUs placed on the torso, right arm, left arm, right leg, and left leg.

The \textit{UTD-MHAD} dataset (2015) \cite{chen2015utd} captured 27 diverse human actions, including 20 upper-body and 7 lower-body motions, by using both a Kinect camera and a wearable inertial sensor positioned either on the subject's wrist or thigh. The Kinect camera records high-resolution color and depth images at 30 frames per second, while the inertial sensor captures precise motion data, including acceleration, angular velocity, and magnetic strength, at a sampling rate of 50 Hz.1

The \textit{RealWorld} dataset (2016) \cite{sztyler2016body} collected data from 15 participants engaged in 7 activities, including climbing stairs, jumping, lying, standing, sitting, running/jogging, and walking. Recorded via smartphones and smartwatches positioned at 7 body locations, the dataset offers accelerometer and gyroscope data sampled at \SI{50}{\hertz}, with each activity performed for 10 minutes (except jumping, approximately 1.7 minutes). 

The \textit{ActiveMiles} dataset (2016) \cite{ravi2016deep}

The \textit{Mobiact} dataset (2016) \cite{vavoulas2016mobiact}

The \textit{SBHAR} dataset (2016) \cite{reyes2016transition} provides approximately 5 hours of smartphone-based data with activity labels and user information, involving 30 users aged 19 to 48. Participants wore smartphones on their waists and performed 12 distinct activities according to a predefined protocol, with data collected from built-in accelerometers and gyroscopes and labeled with both activity and user identifiers. 

The \textit{UCI Smartphone} dataset (2017) \cite{almaslukh2017effective}

The \textit{DeepSense} dataset (2017) \cite{yao2017deepsense}

The \textit{MotionSense} dataset (2018) \cite{malekzadeh2018motionsense}

The \textit{SHL} dataset (2018) \cite{gjoreski2018university} was recorded over 7 months in 2017 by 3 participants in the UK, comprises 750 hours of labeled locomotion data from 8 transportation modes, captured using a body-worn camera and 4 smartphones, providing multi-modal insights into real-life mobile user behavior. 

The \textit{MM-fit} dataset (2020) \cite{stromback2020mmfit} contains 11 workout activities, capturing 2D and 3D skeletal poses along with five IMUs from commercial mobile devices (earbud, smartphone, smartwatch) across 21 workout sessions. %Each session comprises three sets, each containing ten exercises and repetitions, with continuous recording during rest intervals to capture natural behavior. 

The Capture-24 dataset (2021) \cite{chan2021capture}

UK-Biobank data source (2023) ???\cite{yuan2024self}



\begin{table}[ht]
\footnotesize
    \centering
    \caption{Evaluation dataset information for our experiments}
    
    \footnotesize
    \begin{tabular}{ccccccc}
        \toprule
        Dataset & Subjects & Application & Sensor & Position & \# Classes & Frequency (Hz) \\
        \midrule
        WISDM & 36 & Locomotion & 3D Acc. & pants pocket & 6 & 20 \\
        MHEALTH & 10 & ADL & 3D Acc. + 9D IMU & chest - ankle - arm & 12 & 50 \\ 
        Opportunity & 4 & Locomotion & 9D IMU & back and limbs & 5 & 30 \\
        Opportunity & 4 & Gesture & 9D IMU & back and limbs & 18 & 30 \\
        PAMAP2 & 8 & ADL & 9D IMU + & hand-chest-ankle & 13 & 50 \\
        MM-Fit & 10 & Physical exercises & 6D IMU & ear - wrists - waists & 11 & 50 \\ 
        MotionSense & 24 & Locomotion & 6D IMU + & front pocket & 6 & 50 \\
        \bottomrule
    \end{tabular}
    \label{tab:datasets}
\end{table}
